Direct Multi-Turn Preference Optimization for Language Agents

Adapting Large Language Models (LLMs) for agent tasks is critical in developing language agents. Direct Preference Optimization (DPO) is a promising technique for this adaptation with the alleviation of compounding errors, offering a means to directly optimize Reinforcement Learning (RL) objectives. However, applying DPO to multi-turn tasks presents challenges due to the inability to cancel the partition function. Overcoming this obstacle involves making the partition function independent of the current state and addressing length disparities between preferred and dis-preferred trajectories. In this light, we replace the policy constraint with the state-action occupancy measure constraint in the RL objective and add length normalization to the Bradley-Terry model, yielding a novel loss function named DMPO for multi-turn agent tasks with theoretical explanations. Extensive experiments on three multi-turn agent task datasets confirm the effectiveness and superiority of the DMPO loss. The code is available at https://github.com/swt-user/DMPO.

==> backup/1_Introduction_0612.tex <==
\section{Introduction}

% Since the advent of artificial intelligence, the pursuit of creating generalist agents capable of solving and adapting to complex tasks has been a primary objective~\cite{DBLP:journals/tmlr/ReedZPCNBGSKSEBREHCHVBF22, DBLP:journals/corr/abs-2404-10179}. Recently Large Language Models (LLMs) have demonstrated significant potential in tackling intricate tasks through instruction following~\cite{DBLP:conf/nips/Ouyang0JAWMZASR22}, action planning~\cite{DBLP:conf/icml/HuangAPM22}, and tool utilization~\cite{DBLP:conf/nips/SchickDDRLHZCS23}, giving rise to a novel research direction of \textit{language agents}~\cite{DBLP:conf/iclr/YaoZYDSN023}. 
% % Projects such as AutoGPT~\cite{}, BabyAGI~\cite{}, xx, have employed language agents in a wide array of real-world domains. 
% Despite the significant successes thus far, there exists significant potential for future advancements due to the substantial domain gap between the pretraining tasks of LLMs and the agent tasks.
%%% FFL 0612 %%% 
Pursuing generalist agents capable of solving and adapting to complex tasks has been a primary objective in the artificial intelligence community~\cite{DBLP:journals/tmlr/ReedZPCNBGSKSEBREHCHVBF22, DBLP:journals/corr/abs-2404-10179}. \textit{Language agents}~\cite{DBLP:conf/iclr/YaoZYDSN023} become an emerging research direction in recent years owing to the significant potential of Large Language Models in tackling intricate tasks through instruction following~\cite{DBLP:conf/nips/Ouyang0JAWMZASR22}, action planning~\cite{DBLP:conf/icml/HuangAPM22}, and tool utilization~\cite{DBLP:conf/nips/SchickDDRLHZCS23}. 
Nevertheless, there exists significant potential for future advancements of language agents due to the substantial gap between the pretraining task of LLMs and agent tasks.

Behavioral Cloning (BC)~\cite{DBLP:journals/neco/Pomerleau91} is a commonly used approach to bridge the domain gap by fine-tuning LLMs through expert agent trajectories. For instance, recent efforts on BC~\cite{DBLP:journals/corr/abs-2310-05915, DBLP:journals/corr/abs-2310-12823, DBLP:journals/corr/abs-2311-05657} perform Supervised Fine-tuning (SFT) of LLMs on optimal state-action pairs. While these methods can rapidly adapt LLMs to agent tasks, BC is significantly affected by \textit{compounding errors} - minor errors of the learner will accumulate along interactions between the agent and environment, leading to performance deterioration in non-deterministic environments~\cite{DBLP:journals/jmlr/RossGB11}. 

% To bridge the domain gap, a commonly used approach involves fine-tuning the LLMs through expert agent trajectories, known as Behavioral Cloning (BC)~\cite{DBLP:journals/neco/Pomerleau91}. Recent efforts~\cite{DBLP:journals/corr/abs-2310-05915, DBLP:journals/corr/abs-2310-12823, DBLP:journals/corr/abs-2311-05657} have utilized BC methods to perform Supervised Fine-tuning (SFT) of LLMs on optimal state-action pairs. While these methods can rapidly adapt LLMs to agent tasks, BC is significantly affected by \textit{compounding errors} - the minor errors of the learners can accumulate over time, leading to performance deterioration in non-deterministic environments.~\cite{DBLP:journals/jmlr/RossGB11}. 
% % However, BC heavily relies on the quality of expert data and is significantly affected by compounding errors in non-deterministic environments~\cite{DBLP:journals/jmlr/RossGB11}. 

% To mitigate the impact of compounding errors, some works~\cite{DBLP:journals/corr/abs-2312-14878, DBLP:journals/corr/abs-2404-01663} refine the LLMs using classical Reinforcement Learning approaches, such as Proximal Policy Optimization (PPO)~\cite{DBLP:journals/corr/SchulmanWDRK17}. This necessitates continuous interaction with the environment during training, leading to challenges like training instability~\cite{}. In contrast, alternative methodologies like Direct Preference Optimization (DPO)~\cite{DBLP:conf/nips/RafailovSMMEF23} have garnered significant interest due to their simple implementation and robustness, enabling the optimization of RL-based objectives using a simple binary cross-entropy objective. \citet{DBLP:journals/corr/abs-2403-02502} has employed the DPO loss function to enhance LLMs' performance in agent tasks. However, the DPO loss is specifically designed for the single-turn bandit setting and unsuitable for multi-turn agent tasks, resulting in suboptimal performance.

% Direct Preference Optimization (DPO)~\cite{DBLP:conf/nips/RafailovSMMEF23}, which directly optimizes the Reinforcement Learning (RL) objectives and mitigates the compounding errors, has achieved remarkable success in the single-turn preference alignment task. Its simple and robust implementation alleviates the necessity for continuous interaction with the environment and the training instability inherent in traditional RL algorithms~\cite{DBLP:journals/corr/abs-2312-14878, DBLP:journals/corr/abs-2404-01663}. \citet{DBLP:journals/corr/abs-2403-02502} has employed the DPO loss to enhance LLMs' performance in agent tasks. However, the DPO loss is tailored specifically for the single-turn bandit setting and is ill-suited for multi-turn agent tasks, leading to suboptimal performance.

% In addressing the compounding errors, Direct Preference Optimization (DPO)~\cite{DBLP:conf/nips/RafailovSMMEF23} has achieved remarkable success in the single-turn preference alignment due to its simple implementation and robustness. DPO optimizes the Reinforcement Learning (RL) objectives using a simple binary cross-entropy objective, alleviating the necessity for continuous interaction with the environment and the training instability of traditional RL algorithms~\cite{DBLP:journals/corr/abs-2312-14878, DBLP:journals/corr/abs-2404-01663}. \citet{DBLP:journals/corr/abs-2403-02502} has employed the DPO loss to enhance LLMs' performance in agent tasks. However, the DPO loss is tailored specifically for the single-turn bandit setting and is ill-suited for multi-turn agent tasks, leading to suboptimal performance.
%%% FFL 0612 %%%
In addressing the compounding errors, Direct Preference Optimization~\cite{DBLP:conf/nips/RafailovSMMEF23} has achieved remarkable success in the single-turn preference alignment due to its simple implementation and robustness. DPO optimizes the Reinforcement Learning (RL) objectives using a simple binary cross-entropy objective, alleviating the necessity for continuous interaction with the environment and the training instability of traditional RL algorithms~\cite{DBLP:journals/corr/abs-2312-14878, DBLP:journals/corr/abs-2404-01663}. \citet{DBLP:journals/corr/abs-2403-02502} has employed the DPO loss to enhance LLMs' performance in agent tasks. However, the DPO loss is tailored specifically for the single-turn bandit setting and is ill-suited for multi-turn agent tasks, leading to suboptimal performance.

This work aims to develop a robust loss function capable of directly optimizing RL objectives in multi-turn scenarios. The key to achieving this goal lies in eliminating the partition function in the Bradley-Terry (BT) model~\cite{xxx}. 
To achieve this, we need to make the partition function independent of the current state and eliminate the effect of length difference between XXX and XXX trajectories.
In this light, we replace the policy constraint with the state-action occupancy measure (SAOM) constraint in the RL objective and add length normalization to the BT model.
These modifications allowing us to obtain a new and simple loss function DMPO for multi-turn agent tasks. 
The state-action occupancy measure describes the distribution of state-action pairs that an agent visits in the space with policy~\cite{DBLP:journals/ijon/JohnsonLC00}. Intuitively, by leveraging the novel constraint, the LLMs can mitigate compounding errors by ensuring that they do not deviate significantly from the reference model, even in unobserved states within the dataset~\cite{DBLP:conf/nips/XuLY20}. Furthermore, we provide a theoretical explanation for the effectiveness of the widely used length normalization trick~\cite{meng2024simpo}. In the RL objective with the SAOM constraint, the length normalization cancels out the partition function from the Bradley-Terry (BT) model~\cite{19ff28b9-64f9-3656-ba40-08326a05748e, DBLP:conf/nips/ChristianoLBMLA17}, resulting in improved performance. 

% Inspired by the success of DPO, our objective is to develop a robust loss function capable of directly optimizing RL objectives in multi-turn scenarios. The key lies in eliminating the partition function in the Bradley-Terry (BT) model. To achieve this, we replace the policy constraint with the state-action occupancy measure (SAOM) constraint in the RL objective. This modification makes the partition function independent of the current state, allowing us to cancel it out and obtain a new and simple loss function DMPO for multi-turn agent tasks. The state-action occupancy measure describes the distribution of state-action pairs that an agent visits in the space with policy~\cite{DBLP:journals/ijon/JohnsonLC00}. Intuitively, by leveraging the novel constraint, the LLMs can mitigate compounding errors by ensuring that they do not deviate significantly from the reference model, even in unobserved states within the dataset~\cite{DBLP:conf/nips/XuLY20}. Furthermore, we provide a theoretical explanation for the effectiveness of the widely used length normalization trick~\cite{meng2024simpo}. In the RL objective with the SAOM constraint, the length normalization cancels out the partition function from the Bradley-Terry (BT) model~\cite{19ff28b9-64f9-3656-ba40-08326a05748e, DBLP:conf/nips/ChristianoLBMLA17}, resulting in improved performance. 

To summarise, our contributions are three folds:
\begin{itemize}[leftmargin=*]
    % \item We introduce a simple loss function called DMPO, aimed at optimizing the RL objective directly in multi-turn scenarios, thereby mitigating the compounding errors associated with BC methods.
    \item We introduce a new loss function called DMPO, which optimizes the RL objective directly in multi-turn scenarios, thereby mitigating the compounding errors associated with BC methods.
    \item We provide a theoretical explanation for the effectiveness of the length normalization trick, demonstrating how it cancels out the partition function in the BT model and improves the performance.
    \item Extensive experiments on three multi-turn agent tasks validate the effectiveness and the superiority of the DMPO loss function.
\end{itemize}
